Suppressing Noise from Built Environment Datasets to Reduce Communication Rounds for Convergence of Federated Learning

Smart sensing provides an easier and convenient data-driven mechanism for monitoring and control in the built environment. Data generated in the built environment are privacy sensitive and limited. Federated learning is an emerging paradigm that provides privacy-preserving collaboration among multiple participants for model training without sharing private and limited data. The noisy labels in the datasets of the participants degrade the performance and increase the number of communication rounds for convergence of federated learning. Such large communication rounds require more time and energy to train the model. In this paper, we propose a federated learning approach to suppress the unequal distribution of the noisy labels in the dataset of each participant. The approach first estimates the noise ratio of the dataset for each participant and normalizes the noise ratio using the server dataset. The proposed approach can handle bias in the server dataset and minimizes its impact on the participants' dataset. Next, we calculate the optimal weighted contributions of the participants using the normalized noise ratio and influence of each participant. We further derive the expression to estimate the number of communication rounds required for the convergence of the proposed approach. Finally, experimental results demonstrate the effectiveness of the proposed approach over existing techniques in terms of the communication rounds and achieved performance in the built environment.

==> 1/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.7,0.65;
#set pointsize 1.5;
set xlabel '{\textbf{Noise ratio}}' offset 1;
set ylabel '{\textbf{Local accuracy (in \%)}}' offset 1;
set pointsize 2;
set ytics ('25' 25,'50' 50,'75' 75, '100' 100)
set xtics ('0.0' 0.0,'0.2' 0.2, '0.4' 0.4,'0.6' 0.6,'0.8' 0.8)
#set grid
#set arrow 1  from 160,91 to 185,88  
#set key right bottom Right horizontal vertical
set key at 40,26 right bottom horizontal samplen 3  width 2
#set object 1 ellipse center 160,92 size 55, 2.5 angle 0 front fc rgb"green" behind fs solid 0.7
#set label 'accuracy' at 35,94;
#set label 'Stability stage' at 152,87;

plot [0.0:0.80][20:100] 'final_out_d1' using 1:2 with lines lt 4 lc rgb "#006400" lw 4 title '$\mathbf{10\%}$','final_out_d1' using 1:2:($3):($4) lt 1 lc rgb "#006400" lw 4 notitle with yerrorbars, 'final_out_d1' using 1:3 with lines lt 6 lc rgb "#000064" lw 4 title '$\mathbf{20\%}$', 'final_out_d1' using 1:3:($8):($9) lt 1 lc rgb "#000064" lw 4 notitle with yerrorbars, 'final_out_d1' using 1:4 with lines lt 8 lc rgb "magenta" lw 4 title '$\mathbf{30\%}$', 'final_out_d1' using 1:4:($10):($11) lt 1 lc rgb "magenta" lw 4 notitle with yerrorbars,'final_out_d1' using 1:5 with lines lt 5 lc rgb "#654321" lw 4 title '$\mathbf{40\%}$','final_out_d1' using 1:5:($12):($13) lt 1 lc rgb "#654321" lw 4 notitle with yerrorbars,


==> 1/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3276.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,851){\makebox(0,0)[r]{\strut{}25}}%
      \put(814,1586){\makebox(0,0)[r]{\strut{}50}}%
      \put(814,2320){\makebox(0,0)[r]{\strut{}75}}%
      \put(814,3055){\makebox(0,0)[r]{\strut{}100}}%
      \put(946,484){\makebox(0,0){\strut{}0.0}}%
      \put(1870,484){\makebox(0,0){\strut{}0.2}}%
      \put(2795,484){\makebox(0,0){\strut{}0.4}}%
      \put(3719,484){\makebox(0,0){\strut{}0.6}}%
      \put(4643,484){\makebox(0,0){\strut{}0.8}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,1879){\rotatebox{-270}{\makebox(0,0){\textbf{Local accuracy (in \%)}}}}%
      \put(2926,154){\makebox(0,0){\textbf{Noise ratio}}}%
      \csname LTb\endcsname%%
      \put(183426,1210){\makebox(0,0)[r]{\strut{}$\mathbf{10\%}$}}%
      \csname LTb\endcsname%%
      \put(183426,990){\makebox(0,0)[r]{\strut{}$\mathbf{20\%}$}}%
      \csname LTb\endcsname%%
      \put(185073,1210){\makebox(0,0)[r]{\strut{}$\mathbf{30\%}$}}%
      \csname LTb\endcsname%%
      \put(185073,990){\makebox(0,0)[r]{\strut{}$\mathbf{40\%}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 1/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 1/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 4/21/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 0.9,0.8;
set ylabel '\large \textbf{Local F1-score}' offset 1.0;
set xlabel '\large \textbf{Noise ratio}' offset 0.0;

set xtics ('0.1' 1, '0.2' 2, '0.3' 3, '0.4' 4, '0.5'5,'0.6'6)
set ytics ('30'30,'50'50,'70'70,'90'90)  
#set grid

Theads = 'heads size 0.10,90 front ls 238 lc rgb "black" lw 5'
set arrow 1 from 0.85,90.13 to 0.85,94.02 @Theads
set arrow 2 from 1.15,89.43 to 1.15,93.79 @Theads

set arrow 3 from 1.85,86.42 to 1.85,90.29 @Theads
set arrow 4 from 2.15,85.21 to 2.15,89.81 @Theads

set arrow 5 from 2.85,79.61 to 2.85,84.20 @Theads
set arrow 6 from 3.15,76.42 to 3.15,80.80 @Theads

set arrow 7 from 3.85,71.22 to 3.85,77.29 @Theads
set arrow 8 from 4.15,66.39 to 4.15,72.42 @Theads

set arrow 9 from  4.85,62.63 to 4.85,68.21 @Theads
set arrow 10 from 5.15,58.11 to 5.15,64.57 @Theads

set arrow 11 from  5.85,50.13 to 5.85,55.67 @Theads
set arrow 12 from 6.15,45.21 to 6.15,53.20 @Theads

set object 1 ellipse center 1.0,92 size 1,5 angle 0 front fc rgb"green" behind fs solid 0.6
set object 2 ellipse center 6,50 size 1,6 angle 0 front fc rgb"green" behind fs solid 0.6
set arrow from 1.5,92.5 to 2.0,92.5 head nofilled front lt 1 lw 5 lc rgb "black"
set label at 2.1,92.5 '\large \textcolor{blue}{e1}' 

set arrow from 6,53 to 6,65 head nofilled front lt 1 lw 5 lc rgb "black"
set label at 5.85,66.5 '\large \textcolor{blue}{e2}' 

#set key horizontal
set key top horizontal
set boxwidth 0.25 relative
set style fill solid 0.9
plot [0.5:6.5][30:95] "final_out_d1" u ($1-0.15):2 w boxes fill pattern 6 lc rgb "red" lw 4 title '\large LMR', "final_out_d1" u ($1+0.15):3 w boxes fill pattern 2 lc rgb "#21908d" lw 4 title '\large SHL'




==> 4/21/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6480.00,4032.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,704){\makebox(0,0)[r]{\strut{}30}}%
      \put(682,1660){\makebox(0,0)[r]{\strut{}50}}%
      \put(682,2616){\makebox(0,0)[r]{\strut{}70}}%
      \put(682,3572){\makebox(0,0)[r]{\strut{}90}}%
      \put(1253,484){\makebox(0,0){\strut{}0.1}}%
      \put(2131,484){\makebox(0,0){\strut{}0.2}}%
      \put(3009,484){\makebox(0,0){\strut{}0.3}}%
      \put(3888,484){\makebox(0,0){\strut{}0.4}}%
      \put(4766,484){\makebox(0,0){\strut{}0.5}}%
      \put(5644,484){\makebox(0,0){\strut{}0.6}}%
      \put(2219,3692){\makebox(0,0)[l]{\strut{}\large \textcolor{blue}{e1}}}%
      \put(5512,2449){\makebox(0,0)[l]{\strut{}\large \textcolor{blue}{e2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,2257){\rotatebox{-270}{\makebox(0,0){\strut{}\large \textbf{Local F1-score}}}}%
      \put(3448,154){\makebox(0,0){\strut{}\large \textbf{Noise ratio}}}%
      \csname LTb\endcsname%%
      \put(3581,3638){\makebox(0,0)[r]{\strut{}\large LMR}}%
      \csname LTb\endcsname%%
      \put(5096,3638){\makebox(0,0)[r]{\strut{}\large SHL}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 4/21/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 4/21/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 4/22/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 0.9,0.8;
set ylabel '\large \textbf{Global F1-score}' offset 1.0;
set xlabel '\large \textbf{Noise ratio}' offset 0.0;

set xtics ('0.1' 1, '0.2' 2, '0.3' 3, '0.4' 4, '0.5'5,'0.6'6)
set ytics ('20'20,'40'40,'60'60,'80'80)  
#set grid

Theads = 'heads size 0.10,90 front ls 238 lc rgb "black" lw 5'
set arrow 1 from 0.85,83.71 to 0.85,87.38 @Theads
set arrow 2 from 1.15,82.17 to 1.15,87.21 @Theads

set arrow 3 from 1.85,78.21 to 1.85,83.22 @Theads
set arrow 4 from 2.15,76.11 to 2.15,81.21 @Theads

set arrow 5 from 2.85,70.31 to 2.85,77.91 @Theads
set arrow 6 from 3.15,67.44 to 3.15,73.21 @Theads

set arrow 7 from 3.85,63.32 to 3.85,70.28 @Theads
set arrow 8 from 4.15,61.22 to 4.15,68.42 @Theads

set arrow 9 from  4.85,53.49 to 4.85,62.44 @Theads
set arrow 10 from 5.15,51.89 to 5.15,58.43 @Theads

set arrow 11 from  5.85,36.81 to 5.85,44.57 @Theads
set arrow 12 from 6.15,30.22 to 6.15,39.26 @Theads



#set key horizontal
set key top horizontal
set boxwidth 0.25 relative
set style fill solid 0.9
plot [0.5:6.5][20:90] "final_out_d1" u ($1-0.15):2 w boxes fill pattern 6 lc rgb "red" lw 4 title '\large LMR', "final_out_d1" u ($1+0.15):3 w boxes fill pattern 2 lc rgb "#21908d" lw 4 title '\large SHL'




==> 4/22/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6480.00,4032.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,704){\makebox(0,0)[r]{\strut{}20}}%
      \put(682,1592){\makebox(0,0)[r]{\strut{}40}}%
      \put(682,2479){\makebox(0,0)[r]{\strut{}60}}%
      \put(682,3367){\makebox(0,0)[r]{\strut{}80}}%
      \put(1253,484){\makebox(0,0){\strut{}0.1}}%
      \put(2131,484){\makebox(0,0){\strut{}0.2}}%
      \put(3009,484){\makebox(0,0){\strut{}0.3}}%
      \put(3888,484){\makebox(0,0){\strut{}0.4}}%
      \put(4766,484){\makebox(0,0){\strut{}0.5}}%
      \put(5644,484){\makebox(0,0){\strut{}0.6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,2257){\rotatebox{-270}{\makebox(0,0){\strut{}\large \textbf{Global F1-score}}}}%
      \put(3448,154){\makebox(0,0){\strut{}\large \textbf{Noise ratio}}}%
      \csname LTb\endcsname%%
      \put(3581,3638){\makebox(0,0)[r]{\strut{}\large LMR}}%
      \csname LTb\endcsname%%
      \put(5096,3638){\makebox(0,0)[r]{\strut{}\large SHL}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 4/22/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 4/22/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 5/31/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 0.9,0.8;
set ylabel '\large \textbf{Contribution ratio}' offset 1.0;
set xlabel '\large \textbf{Noise ratio}' offset 0.0;

set xtics ('0.1' 1, '0.2' 2, '0.3' 3, '0.4' 4, '0.5'5,'0.6'6)
set ytics ('0.2'0.2,'0.6'0.6,'1.0'1.0)  


#set key horizontal
set key top horizontal
set boxwidth 0.25 relative
set style fill solid 0.9
plot [0.3:6.7][0:1.2] "final_out_d1" u ($1-0.25):2 w boxes fill pattern 6 lc rgb "red" lw 4 title '\large $\mathbf{S_1}$', "final_out_d1" u ($1+0.05):3 w boxes fill pattern 2 lc rgb "#21908d" lw 4 title '\large $\mathbf{S_2}$', "final_out_d1" u ($1+0.35):4 w boxes fill pattern 9 lc rgb "#000064" lw 4 title '\large $\mathbf{S_3}$'




==> 5/31/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6480.00,4032.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,1222){\makebox(0,0)[r]{\strut{}0.2}}%
      \put(814,2258){\makebox(0,0)[r]{\strut{}0.6}}%
      \put(814,3293){\makebox(0,0)[r]{\strut{}1.0}}%
      \put(1508,484){\makebox(0,0){\strut{}0.1}}%
      \put(2311,484){\makebox(0,0){\strut{}0.2}}%
      \put(3113,484){\makebox(0,0){\strut{}0.3}}%
      \put(3916,484){\makebox(0,0){\strut{}0.4}}%
      \put(4718,484){\makebox(0,0){\strut{}0.5}}%
      \put(5521,484){\makebox(0,0){\strut{}0.6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,2257){\rotatebox{-270}{\makebox(0,0){\strut{}\large \textbf{Contribution ratio}}}}%
      \put(3514,154){\makebox(0,0){\strut{}\large \textbf{Noise ratio}}}%
      \csname LTb\endcsname%%
      \put(2066,3638){\makebox(0,0)[r]{\strut{}\large $\mathbf{S_1}$}}%
      \csname LTb\endcsname%%
      \put(3581,3638){\makebox(0,0)[r]{\strut{}\large $\mathbf{S_2}$}}%
      \csname LTb\endcsname%%
      \put(5096,3638){\makebox(0,0)[r]{\strut{}\large $\mathbf{S_3}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 5/31/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 5/31/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 5/32/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 0.9,0.8;
set ylabel '\large \textbf{Contribution ratio}' offset 1.0;
set xlabel '\large \textbf{Noise ratio}' offset 0.0;

set xtics ('0.1' 1, '0.2' 2, '0.3' 3, '0.4' 4, '0.5'5,'0.6'6)
set ytics ('0.2'0.2,'0.6'0.6,'1.0'1.0)  


#set key horizontal
set key top horizontal
set boxwidth 0.25 relative
set style fill solid 0.9
plot [0.3:6.7][0:1.2] "final_out_d1" u ($1-0.25):2 w boxes fill pattern 6 lc rgb "red" lw 4 title '\large $\mathbf{S_1}$', "final_out_d1" u ($1+0.05):3 w boxes fill pattern 2 lc rgb "#21908d" lw 4 title '\large $\mathbf{S_2}$', "final_out_d1" u ($1+0.35):4 w boxes fill pattern 9 lc rgb "#000064" lw 4 title '\large $\mathbf{S_3}$'




==> 5/32/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6480.00,4032.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,1222){\makebox(0,0)[r]{\strut{}0.2}}%
      \put(814,2258){\makebox(0,0)[r]{\strut{}0.6}}%
      \put(814,3293){\makebox(0,0)[r]{\strut{}1.0}}%
      \put(1508,484){\makebox(0,0){\strut{}0.1}}%
      \put(2311,484){\makebox(0,0){\strut{}0.2}}%
      \put(3113,484){\makebox(0,0){\strut{}0.3}}%
      \put(3916,484){\makebox(0,0){\strut{}0.4}}%
      \put(4718,484){\makebox(0,0){\strut{}0.5}}%
      \put(5521,484){\makebox(0,0){\strut{}0.6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,2257){\rotatebox{-270}{\makebox(0,0){\strut{}\large \textbf{Contribution ratio}}}}%
      \put(3514,154){\makebox(0,0){\strut{}\large \textbf{Noise ratio}}}%
      \csname LTb\endcsname%%
      \put(2066,3638){\makebox(0,0)[r]{\strut{}\large $\mathbf{S_1}$}}%
      \csname LTb\endcsname%%
      \put(3581,3638){\makebox(0,0)[r]{\strut{}\large $\mathbf{S_2}$}}%
      \csname LTb\endcsname%%
      \put(5096,3638){\makebox(0,0)[r]{\strut{}\large $\mathbf{S_3}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 5/32/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 5/32/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 5/33/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 0.9,0.8;
set ylabel '\large \textbf{Local F1-score}' offset 1.0;
set xlabel '\large \textbf{Noise ratio}' offset 0.0;

set xtics ('0.1' 1, '0.2' 2, '0.3' 3, '0.4' 4, '0.5'5,'0.6'6)
set ytics ('40'40,'60'60,'80'80)  

Theads = 'heads size 0.10,90 front ls 238 lc rgb "black" lw 5'
set arrow 1 from 0.75,87.5 to 0.75,91.44 @Theads
set arrow 2 from 1.05,88.21 to 1.05,92.37 @Theads
set arrow 3 from 1.35,90.43 to 1.35,94.23 @Theads

set arrow 4 from 1.75,79.41 to 1.75,83.46 @Theads
set arrow 5 from 2.05,84.21 to 2.05,88.91 @Theads
set arrow 6 from 2.35,86.13 to 2.35,91.01 @Theads

set arrow 7 from 2.75,67.43 to 2.75,73.41 @Theads
set arrow 8 from 3.05,72.31 to 3.05,78.44 @Theads
set arrow 9 from 3.35,77.41 to 3.35,84.43 @Theads

set arrow 10 from 3.75,60.17 to 3.75,66.41 @Theads
set arrow 11 from 4.05,65.42 to 4.05,73.41 @Theads
set arrow 12 from 4.35,70.22 to 4.35,77.47 @Theads

set arrow 13 from 4.75,50.17 to 4.75,58.27 @Theads
set arrow 14 from 5.05,53.41 to 5.05,62.22 @Theads
set arrow 15 from 5.35,61.47 to 5.35,69.51 @Theads

set arrow 16 from 5.75,36.34 to 5.75,45.29 @Theads
set arrow 17 from 6.05,45.93 to 6.05,54.79 @Theads
set arrow 18 from 6.35,48.79 to 6.35,56.71 @Theads



#set key horizontal
set key top vertical
set boxwidth 0.25 relative
set style fill solid 0.9
plot [0.3:6.7][30:95] "final_out_d1" u ($1-0.25):2 w boxes fill pattern 6 lc rgb "red" lw 4 title '\large $\mathbf{S_1}$', "final_out_d1" u ($1+0.05):3 w boxes fill pattern 2 lc rgb "#21908d" lw 4 title '\large $\mathbf{S_2}$', "final_out_d1" u ($1+0.35):4 w boxes fill pattern 9 lc rgb "#000064" lw 4 title '\large $\mathbf{S_3}$'




==> 5/33/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6480.00,4032.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,1182){\makebox(0,0)[r]{\strut{}40}}%
      \put(682,2138){\makebox(0,0)[r]{\strut{}60}}%
      \put(682,3094){\makebox(0,0)[r]{\strut{}80}}%
      \put(1390,484){\makebox(0,0){\strut{}0.1}}%
      \put(2214,484){\makebox(0,0){\strut{}0.2}}%
      \put(3037,484){\makebox(0,0){\strut{}0.3}}%
      \put(3860,484){\makebox(0,0){\strut{}0.4}}%
      \put(4683,484){\makebox(0,0){\strut{}0.5}}%
      \put(5507,484){\makebox(0,0){\strut{}0.6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,2257){\rotatebox{-270}{\makebox(0,0){\strut{}\large \textbf{Local F1-score}}}}%
      \put(3448,154){\makebox(0,0){\strut{}\large \textbf{Noise ratio}}}%
      \csname LTb\endcsname%%
      \put(5096,3638){\makebox(0,0)[r]{\strut{}\large $\mathbf{S_1}$}}%
      \csname LTb\endcsname%%
      \put(5096,3418){\makebox(0,0)[r]{\strut{}\large $\mathbf{S_2}$}}%
      \csname LTb\endcsname%%
      \put(5096,3198){\makebox(0,0)[r]{\strut{}\large $\mathbf{S_3}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 5/33/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 5/33/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 5/34/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex';
set size 0.9,0.8;
set ylabel '\large \textbf{Local F1-score}' offset 1.0;
set xlabel '\large \textbf{Noise ratio}' offset 0.0;

set xtics ('0.1' 1, '0.2' 2, '0.3' 3, '0.4' 4, '0.5'5,'0.6'6)
set ytics ('40'40,'60'60,'80'80)  

Theads = 'heads size 0.10,90 front ls 238 lc rgb "black" lw 5'
set arrow 1 from 0.75,85.43 to 0.75,89.25 @Theads
set arrow 2 from 1.05,87.11 to 1.05,91.67 @Theads
set arrow 3 from 1.35,89.43 to 1.35,93.22 @Theads

set arrow 4 from 1.75,78.73 to 1.75,82.39 @Theads
set arrow 5 from 2.05,83.48 to 2.05,87.81 @Theads
set arrow 6 from 2.35,85.41 to 2.35,89.29 @Theads

set arrow 7 from 2.75,67.21 to 2.75,72.73 @Theads
set arrow 8 from 3.05,71.21 to 3.05,76.29 @Theads
set arrow 9 from 3.35,75.49 to 3.35,80.81 @Theads

set arrow 10 from 3.75,60.17 to 3.75,64.47 @Theads
set arrow 11 from 4.05,63.21 to 4.05,67.37 @Theads
set arrow 12 from 4.35,66.77 to 4.35,70.83 @Theads

set arrow 13 from 4.75,49.37 to 4.75,53.73 @Theads
set arrow 14 from 5.05,54.71 to 5.05,58.27 @Theads
set arrow 15 from 5.35,59.37 to 5.35,63.79 @Theads

set arrow 16 from 5.75,35.21 to 5.75,42.03 @Theads
set arrow 17 from 6.05,41.31 to 6.05,46.20 @Theads
set arrow 18 from 6.35,46.35 to 6.35,51.37 @Theads



#set key horizontal
set key top vertical
set boxwidth 0.25 relative
set style fill solid 0.9
plot [0.3:6.7][30:95] "final_out_d1" u ($1-0.25):2 w boxes fill pattern 6 lc rgb "red" lw 4 title '\large $\mathbf{S_1}$', "final_out_d1" u ($1+0.05):3 w boxes fill pattern 2 lc rgb "#21908d" lw 4 title '\large $\mathbf{S_2}$', "final_out_d1" u ($1+0.35):4 w boxes fill pattern 9 lc rgb "#000064" lw 4 title '\large $\mathbf{S_3}$'




==> 5/34/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6480.00,4032.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,1182){\makebox(0,0)[r]{\strut{}40}}%
      \put(682,2138){\makebox(0,0)[r]{\strut{}60}}%
      \put(682,3094){\makebox(0,0)[r]{\strut{}80}}%
      \put(1390,484){\makebox(0,0){\strut{}0.1}}%
      \put(2214,484){\makebox(0,0){\strut{}0.2}}%
      \put(3037,484){\makebox(0,0){\strut{}0.3}}%
      \put(3860,484){\makebox(0,0){\strut{}0.4}}%
      \put(4683,484){\makebox(0,0){\strut{}0.5}}%
      \put(5507,484){\makebox(0,0){\strut{}0.6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,2257){\rotatebox{-270}{\makebox(0,0){\strut{}\large \textbf{Local F1-score}}}}%
      \put(3448,154){\makebox(0,0){\strut{}\large \textbf{Noise ratio}}}%
      \csname LTb\endcsname%%
      \put(5096,3638){\makebox(0,0)[r]{\strut{}\large $\mathbf{S_1}$}}%
      \csname LTb\endcsname%%
      \put(5096,3418){\makebox(0,0)[r]{\strut{}\large $\mathbf{S_2}$}}%
      \csname LTb\endcsname%%
      \put(5096,3198){\makebox(0,0)[r]{\strut{}\large $\mathbf{S_3}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 5/34/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 5/34/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 6/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.7,0.65;
#set pointsize 1.5;
set xlabel '{\textbf{Global iterations}}' offset 1;
set ylabel '{\textbf{Local accuracy}}' offset 1;
set pointsize 2;
set ytics ('60' 60,'70' 70,'80' 80,'90' 90, '100' 100)
set xtics ('20' 20, '40' 40, '60' 60, '80' 80, '100' 100)
#set grid
#set arrow 1  from 160,91 to 185,88  
set key right bottom Right vertical  
#set key at 40,26 right bottom horizontal samplen 3  width 2
#set object 1 ellipse center 160,92 size 55, 2.5 angle 0 front fc rgb"green" behind fs solid 0.7
#set label 'accuracy' at 35,94;
#set label 'Stability stage' at 152,87;

plot [0:100][50:95] 'final_out_d1' using 1:2 with lines lt 2 lc rgb "red" lw 4 title 'Fed-NL', 'final_out_d1' using 1:3 with lines lt 4 lc rgb "#006400" lw 4 title 'Base1', 'final_out_d1' using 1:4 with lines lt 6 lc rgb "#000064" lw 4 title 'Base2', 'final_out_d1' using 1:5 with lines lt 8 lc rgb "magenta" lw 4 title 'Base3'


==> 6/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3276.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,1226){\makebox(0,0)[r]{\strut{}60}}%
      \put(682,1749){\makebox(0,0)[r]{\strut{}70}}%
      \put(682,2271){\makebox(0,0)[r]{\strut{}80}}%
      \put(682,2794){\makebox(0,0)[r]{\strut{}90}}%
      \put(1580,484){\makebox(0,0){\strut{}20}}%
      \put(2346,484){\makebox(0,0){\strut{}40}}%
      \put(3111,484){\makebox(0,0){\strut{}60}}%
      \put(3877,484){\makebox(0,0){\strut{}80}}%
      \put(4643,484){\makebox(0,0){\strut{}100}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,1879){\rotatebox{-270}{\makebox(0,0){\textbf{Local accuracy}}}}%
      \put(2860,154){\makebox(0,0){\textbf{Global iterations}}}%
      \csname LTb\endcsname%%
      \put(3656,1537){\makebox(0,0)[r]{\strut{}Fed-NL}}%
      \csname LTb\endcsname%%
      \put(3656,1317){\makebox(0,0)[r]{\strut{}Base1}}%
      \csname LTb\endcsname%%
      \put(3656,1097){\makebox(0,0)[r]{\strut{}Base2}}%
      \csname LTb\endcsname%%
      \put(3656,877){\makebox(0,0)[r]{\strut{}Base3}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 6/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 6/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 7/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.7,0.65;
#set pointsize 1.5;
set xlabel '{\textbf{Global iterations}}' offset 1;
set ylabel '{\textbf{Local accuracy}}' offset 1;
set pointsize 2;
set ytics ('60' 60,'70' 70,'80' 80,'90' 90, '100' 100)
set xtics ('20' 20, '40' 40, '60' 60, '80' 80, '100' 100)
#set grid
#set arrow 1  from 160,91 to 185,88  
set key right bottom Right vertical  
#set key at 40,26 right bottom horizontal samplen 3  width 2
#set object 1 ellipse center 160,92 size 55, 2.5 angle 0 front fc rgb"green" behind fs solid 0.7
#set label 'accuracy' at 35,94;
#set label 'Stability stage' at 152,87;

plot [0:100][45:90] 'final_out_d1' using 1:2 with lines lt 2 lc rgb "red" lw 4 title 'Fed-NL', 'final_out_d1' using 1:3 with lines lt 4 lc rgb "#006400" lw 4 title 'Base1', 'final_out_d1' using 1:4 with lines lt 6 lc rgb "#000064" lw 4 title 'Base2', 'final_out_d1' using 1:5 with lines lt 8 lc rgb "magenta" lw 4 title 'Base3'


==> 7/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3276.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,1488){\makebox(0,0)[r]{\strut{}60}}%
      \put(682,2010){\makebox(0,0)[r]{\strut{}70}}%
      \put(682,2533){\makebox(0,0)[r]{\strut{}80}}%
      \put(682,3055){\makebox(0,0)[r]{\strut{}90}}%
      \put(1580,484){\makebox(0,0){\strut{}20}}%
      \put(2346,484){\makebox(0,0){\strut{}40}}%
      \put(3111,484){\makebox(0,0){\strut{}60}}%
      \put(3877,484){\makebox(0,0){\strut{}80}}%
      \put(4643,484){\makebox(0,0){\strut{}100}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,1879){\rotatebox{-270}{\makebox(0,0){\textbf{Local accuracy}}}}%
      \put(2860,154){\makebox(0,0){\textbf{Global iterations}}}%
      \csname LTb\endcsname%%
      \put(3656,1537){\makebox(0,0)[r]{\strut{}Fed-NL}}%
      \csname LTb\endcsname%%
      \put(3656,1317){\makebox(0,0)[r]{\strut{}Base1}}%
      \csname LTb\endcsname%%
      \put(3656,1097){\makebox(0,0)[r]{\strut{}Base2}}%
      \csname LTb\endcsname%%
      \put(3656,877){\makebox(0,0)[r]{\strut{}Base3}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 7/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 7/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 8/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.7,0.65;
#set pointsize 1.5;
set xlabel '{\textbf{Noise ratio}}' offset 1,0.5;
set ylabel '{\textbf{Global iterations}}' offset 1;
set pointsize 2;
set ytics ('50' 50,'100' 100,'150' 150,'200' 200, '250' 250)
set xtics ('0.1' 0.1, '0.2' 0.2, '0.3' 0.3, '0.4' 0.4, '0.5' 0.5, '0.6' 0.6)
#set grid
#set arrow 1  from 160,91 to 185,88  
set key top left vertical  
#set key at 40,26 right bottom horizontal samplen 3  width 2
#set object 1 ellipse center 160,92 size 55, 2.5 angle 0 front fc rgb"green" behind fs solid 0.7
#set label 'accuracy' at 35,94;
#set label 'Stability stage' at 152,87;

plot [0.1:0.6][20:270] \
'final_out_d1' using 1:5:6 with filledcurve fc rgb "#FAEBD7" notitle,\
'final_out_d1' using 1:7:8 with filledcurve fc rgb "#bbffb9" notitle,\
'final_out_d1' using 1:9:10 with filledcurve fc rgb "#e8f4f8" notitle,\
'final_out_d1' using 1:2 with lines lt 2 lc rgb "red" lw 4 title 'E=20', 'final_out_d1' using 1:3 with lines lt 4 lc rgb "#006400" lw 4 title 'E=30', 'final_out_d1' using 1:4 with lines lt 6 lc rgb "#000064" lw 4 title 'E=40','final_out_d1' using 1:11 with points lt 2 lc rgb "red" lw 4 notitle,'final_out_d1' using 1:12 with points lt 4 lc rgb "#006400" lw 4 notitle, 'final_out_d1' using 1:13 with points lt 6 lc rgb "#000064" lw 4 notitle


==> 8/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3276.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,889){\makebox(0,0)[r]{\strut{}50}}%
      \put(814,1382){\makebox(0,0)[r]{\strut{}100}}%
      \put(814,1874){\makebox(0,0)[r]{\strut{}150}}%
      \put(814,2366){\makebox(0,0)[r]{\strut{}200}}%
      \put(814,2858){\makebox(0,0)[r]{\strut{}250}}%
      \put(946,374){\makebox(0,0){\strut{}0.1}}%
      \put(1685,374){\makebox(0,0){\strut{}0.2}}%
      \put(2425,374){\makebox(0,0){\strut{}0.3}}%
      \put(3164,374){\makebox(0,0){\strut{}0.4}}%
      \put(3904,374){\makebox(0,0){\strut{}0.5}}%
      \put(4643,374){\makebox(0,0){\strut{}0.6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,1824){\rotatebox{-270}{\makebox(0,0){\textbf{Global iterations}}}}%
      \put(2926,154){\makebox(0,0){\textbf{Noise ratio}}}%
      \csname LTb\endcsname%%
      \put(1606,2882){\makebox(0,0)[r]{\strut{}E=20}}%
      \csname LTb\endcsname%%
      \put(1606,2662){\makebox(0,0)[r]{\strut{}E=30}}%
      \csname LTb\endcsname%%
      \put(1606,2442){\makebox(0,0)[r]{\strut{}E=40}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 8/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 8/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 9/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.7,0.65;
#set pointsize 1.5;
set xlabel '{\textbf{Noise ratio}}' offset 1,0.5;
set ylabel '{\textbf{Desired precision}}' offset 1;
set pointsize 2;
set ytics ('0.01' 0.01, '0.02' 0.02, '0.03' 0.03, '0.04' 0.04)
set xtics ('0.1' 0.1, '0.2' 0.2, '0.3' 0.3, '0.4' 0.4, '0.5' 0.5, '0.6'0.6)
#set grid
#set arrow 1  from 160,91 to 185,88  
set key top left vertical  
#set key at 40,26 right bottom horizontal samplen 3  width 2
#set object 1 ellipse center 160,92 size 55, 2.5 angle 0 front fc rgb"green" behind fs solid 0.7
#set label 'accuracy' at 35,94;
#set label 'Stability stage' at 152,87;

plot [0.1:0.6][0:0.05] 'final_out_d1' using 1:5:6 with filledcurve fc rgb "#FAEBD7" notitle,\
'final_out_d1' using 1:7:8 with filledcurve fc rgb "#bbffb9" notitle,\
'final_out_d1' using 1:9:10 with filledcurve fc rgb "#e8f4f8" notitle,\
'final_out_d1' using 1:2 with lines lt 2 lc rgb "red" lw 4 title 'R=100', 'final_out_d1' using 1:3 with lines lt 4 lc rgb "#006400" lw 4 title 'R=200', 'final_out_d1' using 1:4 with lines lt 6 lc rgb "#000064" lw 4 title 'R=300','final_out_d1' using 1:11 with points lt 2 lc rgb "red" lw 4 notitle,'final_out_d1' using 1:12 with points lt 4 lc rgb "#006400" lw 4 notitle, 'final_out_d1' using 1:13 with points lt 6 lc rgb "#000064" lw 4 notitle


==> 9/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3276.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,1086){\makebox(0,0)[r]{\strut{}0.01}}%
      \put(946,1578){\makebox(0,0)[r]{\strut{}0.02}}%
      \put(946,2071){\makebox(0,0)[r]{\strut{}0.03}}%
      \put(946,2563){\makebox(0,0)[r]{\strut{}0.04}}%
      \put(1078,374){\makebox(0,0){\strut{}0.1}}%
      \put(1791,374){\makebox(0,0){\strut{}0.2}}%
      \put(2504,374){\makebox(0,0){\strut{}0.3}}%
      \put(3217,374){\makebox(0,0){\strut{}0.4}}%
      \put(3930,374){\makebox(0,0){\strut{}0.5}}%
      \put(4643,374){\makebox(0,0){\strut{}0.6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,1824){\rotatebox{-270}{\makebox(0,0){\textbf{Desired precision}}}}%
      \put(2992,154){\makebox(0,0){\textbf{Noise ratio}}}%
      \csname LTb\endcsname%%
      \put(1870,2882){\makebox(0,0)[r]{\strut{}R=100}}%
      \csname LTb\endcsname%%
      \put(1870,2662){\makebox(0,0)[r]{\strut{}R=200}}%
      \csname LTb\endcsname%%
      \put(1870,2442){\makebox(0,0)[r]{\strut{}R=300}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> 9/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> 9/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> LMR/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.75;
set multi
#set pointsize 1.5;
set xlabel '\large\textbf{Communication rounds}' offset 1;
set ylabel '\large\textbf{Local accuracy (\%)}' offset 1;
set pointsize 1.5;
set ytics ('65'0.65,'70' 0.70,'75'0.75,'80'0.80,'85'0.85,'90'0.90);
set xtics ('0'0,'25'25,'50'50,'75'75,'100'100,'125'125,'150'150,'175'175,'200'200); 
#set key bottom right horizontal
set key bottom vertical right
plot [0:200][0.65:0.95] 'final_out_d1' using 1:2 with lines lt 2 lc rgb "magenta" lw 4 title '\large Base1', 'final_out_d1' using 1:3 with lines lt 2 lc rgb 'blue' lw 4 title '\large Base2','final_out_d1' using 1:4 with lines lt 2 lc rgb "black" lw 4 title '\large Base3', 'final_out_d1' using 1:5 with lines lt 2 lc rgb 'brown' lw 4 title '\large Base4', 'final_out_d1' using 1:6 with lines lt 2 lc rgb 'red' lw 4 title '\large Fed-NL'




==> LMR/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5760.00,3780.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,704){\makebox(0,0)[r]{\strut{}65}}%
      \put(682,1180){\makebox(0,0)[r]{\strut{}70}}%
      \put(682,1656){\makebox(0,0)[r]{\strut{}75}}%
      \put(682,2132){\makebox(0,0)[r]{\strut{}80}}%
      \put(682,2607){\makebox(0,0)[r]{\strut{}85}}%
      \put(682,3083){\makebox(0,0)[r]{\strut{}90}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1383,484){\makebox(0,0){\strut{}25}}%
      \put(1951,484){\makebox(0,0){\strut{}50}}%
      \put(2520,484){\makebox(0,0){\strut{}75}}%
      \put(3089,484){\makebox(0,0){\strut{}100}}%
      \put(3657,484){\makebox(0,0){\strut{}125}}%
      \put(4226,484){\makebox(0,0){\strut{}150}}%
      \put(4794,484){\makebox(0,0){\strut{}175}}%
      \put(5363,484){\makebox(0,0){\strut{}200}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,2131){\rotatebox{-270}{\makebox(0,0){\strut{}\large\textbf{Local accuracy (\%)}}}}%
      \put(3220,154){\makebox(0,0){\strut{}\large\textbf{Communication rounds}}}%
      \csname LTb\endcsname%%
      \put(4376,1757){\makebox(0,0)[r]{\strut{}\large Base1}}%
      \csname LTb\endcsname%%
      \put(4376,1537){\makebox(0,0)[r]{\strut{}\large Base2}}%
      \csname LTb\endcsname%%
      \put(4376,1317){\makebox(0,0)[r]{\strut{}\large Base3}}%
      \csname LTb\endcsname%%
      \put(4376,1097){\makebox(0,0)[r]{\strut{}\large Base4}}%
      \csname LTb\endcsname%%
      \put(4376,877){\makebox(0,0)[r]{\strut{}\large Fed-NL}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> LMR/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> LMR/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> SHL/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.75;
set multi
#set pointsize 1.5;
set xlabel '\large\textbf{Communication rounds}' offset 1;
set ylabel '\large\textbf{Local Accuracy (\%)}' offset 1;
set pointsize 1.5;
set ytics ('65'0.65,'70' 0.70,'75'0.75,'80'0.80,'85'0.85,'90'0.90);
set xtics ('0'0,'25'25,'50'50,'75'75,'100'100,'125'125,'150'150,'175'175,'200'200); 
#set key bottom right horizontal
set key bottom vertical right
plot [0:200][0.65:0.94] 'final_out_d1' using 1:2 with lines lt 2 lc rgb "magenta" lw 4 title '\large Base1', 'final_out_d1' using 1:3 with lines lt 2 lc rgb 'blue' lw 4 title '\large Base2','final_out_d1' using 1:4 with lines lt 2 lc rgb "black" lw 4 title '\large Base3', 'final_out_d1' using 1:5 with lines lt 2 lc rgb 'brown' lw 4 title '\large Base4', 'final_out_d1' using 1:6 with lines lt 2 lc rgb 'red' lw 4 title '\large Fed-NL' 




==> SHL/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5760.00,3780.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,704){\makebox(0,0)[r]{\strut{}65}}%
      \put(682,1196){\makebox(0,0)[r]{\strut{}70}}%
      \put(682,1688){\makebox(0,0)[r]{\strut{}75}}%
      \put(682,2181){\makebox(0,0)[r]{\strut{}80}}%
      \put(682,2673){\makebox(0,0)[r]{\strut{}85}}%
      \put(682,3165){\makebox(0,0)[r]{\strut{}90}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1383,484){\makebox(0,0){\strut{}25}}%
      \put(1951,484){\makebox(0,0){\strut{}50}}%
      \put(2520,484){\makebox(0,0){\strut{}75}}%
      \put(3089,484){\makebox(0,0){\strut{}100}}%
      \put(3657,484){\makebox(0,0){\strut{}125}}%
      \put(4226,484){\makebox(0,0){\strut{}150}}%
      \put(4794,484){\makebox(0,0){\strut{}175}}%
      \put(5363,484){\makebox(0,0){\strut{}200}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,2131){\rotatebox{-270}{\makebox(0,0){\strut{}\large\textbf{Local Accuracy (\%)}}}}%
      \put(3220,154){\makebox(0,0){\strut{}\large\textbf{Communication rounds}}}%
      \csname LTb\endcsname%%
      \put(4376,1757){\makebox(0,0)[r]{\strut{}\large Base1}}%
      \csname LTb\endcsname%%
      \put(4376,1537){\makebox(0,0)[r]{\strut{}\large Base2}}%
      \csname LTb\endcsname%%
      \put(4376,1317){\makebox(0,0)[r]{\strut{}\large Base3}}%
      \csname LTb\endcsname%%
      \put(4376,1097){\makebox(0,0)[r]{\strut{}\large Base4}}%
      \csname LTb\endcsname%%
      \put(4376,877){\makebox(0,0)[r]{\strut{}\large Fed-NL}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> SHL/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> SHL/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> local_epochs/1 <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.7,0.65;
#set pointsize 1.5;
set xlabel '{\textbf{Local epochs}}' offset 1;
set ylabel '{\textbf{Local accuracy (in \%)}}' offset 1;
set pointsize 2;
set ytics ('45' 45,'55' 55,'65' 65, '75' 75,'85' 85,'95' 95)
set xtics ('10' 10, '40' 40, '70' 70, '100' 100, '130' 130,'160' 160, '190' 190,'220' 220)
#set grid
#set arrow 1  from 160,91 to 185,88  
#set key right bottom Right horizontal vertical
set key at 220,36 right bottom horizontal samplen 2.5  width 1.9 spacing 0.9 
#set object 1 ellipse center 160,92 size 55, 2.5 angle 0 front fc rgb"green" behind fs solid 0.7
#set label 'accuracy' at 35,94;
#set label 'Stability stage' at 152,87;

plot [10:220][35:100] 'final_out_d1' using 1:2 with linespoints lt 2 lc rgb "#640000" lw 4 title '$\mathbf{0\%}$', 'final_out_d1' using 1:3 with linespoints lt 4 lc rgb "#006400" lw 4 title '$\mathbf{10\%}$', 'final_out_d1' using 1:4 with linespoints lt 6 lc rgb "#000064" lw 4 title '$\mathbf{20\%}$', 'final_out_d1' using 1:5 with linespoints lt 8 lc rgb "magenta" lw 4 title '$\mathbf{30\%}$', 'final_out_d1' using 1:6 with linespoints lt 10 lc rgb "#654321" lw 4 title '$\mathbf{40\%}$'


==> local_epochs/1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \fontfamily{phv}%
  \fontseries{bx}%
  \selectfont
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3276.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,1066){\makebox(0,0)[r]{\strut{}45}}%
      \put(682,1427){\makebox(0,0)[r]{\strut{}55}}%
      \put(682,1789){\makebox(0,0)[r]{\strut{}65}}%
      \put(682,2151){\makebox(0,0)[r]{\strut{}75}}%
      \put(682,2512){\makebox(0,0)[r]{\strut{}85}}%
      \put(682,2874){\makebox(0,0)[r]{\strut{}95}}%
      \put(814,484){\makebox(0,0){\strut{}10}}%
      \put(1361,484){\makebox(0,0){\strut{}40}}%
      \put(1908,484){\makebox(0,0){\strut{}70}}%
      \put(2455,484){\makebox(0,0){\strut{}100}}%
      \put(3002,484){\makebox(0,0){\strut{}130}}%
      \put(3549,484){\makebox(0,0){\strut{}160}}%
      \put(4096,484){\makebox(0,0){\strut{}190}}%
      \put(4643,484){\makebox(0,0){\strut{}220}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(341,1879){\rotatebox{-270}{\makebox(0,0){\textbf{Local accuracy (in \%)}}}}%
      \put(2860,154){\makebox(0,0){\textbf{Local epochs}}}%
      \csname LTb\endcsname%%
      \put(2419,1235){\makebox(0,0)[r]{\strut{}$\mathbf{0\%}$}}%
      \csname LTb\endcsname%%
      \put(2419,1037){\makebox(0,0)[r]{\strut{}$\mathbf{10\%}$}}%
      \csname LTb\endcsname%%
      \put(2419,839){\makebox(0,0)[r]{\strut{}$\mathbf{20\%}$}}%
      \csname LTb\endcsname%%
      \put(3986,1235){\makebox(0,0)[r]{\strut{}$\mathbf{30\%}$}}%
      \csname LTb\endcsname%%
      \put(3986,1037){\makebox(0,0)[r]{\strut{}$\mathbf{40\%}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> local_epochs/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'


==> local_epochs/c.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5976.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,1131){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(858,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,1984){\makebox(0,0)[r]{\strut{} 1.05}}%
      \put(858,2410){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(858,2837){\makebox(0,0)[r]{\strut{} 1.15}}%
      \put(858,3263){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \put(1564,484){\makebox(0,0){\strut{} 2}}%
      \put(2137,484){\makebox(0,0){\strut{} 4}}%
      \put(2711,484){\makebox(0,0){\strut{} 6}}%
      \put(3285,484){\makebox(0,0){\strut{} 8}}%
      \put(3858,484){\makebox(0,0){\strut{} 10}}%
      \put(4432,484){\makebox(0,0){\strut{} 12}}%
      \put(5005,484){\makebox(0,0){\strut{} 14}}%
      \put(5579,484){\makebox(0,0){\strut{} 16}}%
      \put(352,1983){\rotatebox{-270}{\makebox(0,0){\strut{}\footnotesize {Value of SVM parameter C }}}}%
      \put(3284,154){\makebox(0,0){\strut{}\footnotesize {Accuracy of Lesson 2}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4592,3090){\makebox(0,0)[r]{\strut{}\footnotesize Raw X-axis accelerometer readings}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{c}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> matrix/1_ <==
set terminal epslatex 'phv,bx';
set output '1.tex'; 
set size 0.8,0.8;
set xlabel '\Large{\textbf{Length of MTS (100 - Earliness) (\%)}}' offset 1;
set ylabel '\Large{\textbf{Accuracy (\%)}}' offset 1;
set pointsize 0;
set ytics 0,10,100
#set xtics 0,10,100 

set key left Left box 3

set object 1 ellipse center 88,72 size 30, 10 angle 40 front fc rgb"green" behind fs solid 0.5 lw 1
#set label 'accuracy' at 35,90;
#set label '$(74 \mp 7.5)\%$' at 35,82;


plot [0:100][0:110] 'final_out_d' using 1:6 with linespoints lt 2 lc rgb "red" lw 5 title '\large \boldmath$\alpha=0.5$', 'final_out_d' using 1:5 with linespoints lt 1 lc rgb "blue" lw 5 title '\large \boldmath$\alpha=0.6$', 'final_out_d' using 1:4 with linespoints lt 4 lc rgb "black" lw 5 title '\large \boldmath$\alpha=0.7$', 'final_out_d' using 1:3 with linespoints lt 6 lc rgb "cyan" lw 5 title '\large \boldmath$\alpha=0.8$', 'final_out_d' using 1:2 with linespoints lt 5 lc rgb "magenta" lw 5 title '\large \boldmath$\alpha=0.9$'

